Can Language Models Make Fun? A Case Study in Chinese Comical Crosstalk

Language is the principal tool for human communication, in which humor is one of the most attractive parts. Producing natural language like humans using computers, a.k.a, Natural Language Generation (NLG), has been widely used for dialogue systems, chatbots, machine translation, as well as computer-aid creation e.g., idea generations, scriptwriting. However, the humor aspect of natural language is relatively under-investigated, especially in the age of pre-trained language models. In this work, we aim to preliminarily test whether NLG can generate humor as humans do. We build a new dataset consisting of numerous digitized Chinese Comical Crosstalk scripts (called C$^3$ in short), which is for a popular Chinese performing art called `Xiangsheng' since 1800s. (For convenience for non-Chinese speakers, we called `crosstalk' for `Xiangsheng' in this paper.) We benchmark various generation approaches including training-from-scratch Seq2seq, fine-tuned middle-scale PLMs, and large-scale PLMs (with and without fine-tuning). Moreover, we also conduct a human assessment, showing that 1) large-scale pretraining largely improves crosstalk generation quality; and 2) even the scripts generated from the best PLM is far from what we expect, with only 65% quality of human-created crosstalk. We conclude, humor generation could be largely improved using large-scaled PLMs, but it is still in its infancy. The data and benchmarking code is publicly available in \url{https://github.com/anonNo2/crosstalk-generation}.

==> sub/RAVEN-xiaokang.tex <==
	RAVEN for Train Data Only									
	CPM_large	gpt_ep50	gpt3_base	gpt3_finetune	pangu_a	rnn	smallt5-95	t5	unilm	zhouwenwang
1	0.04855	0	0.00378	0.00076	0.00754	0	0	0	0.00047	0.07012
2	0.23114	0.00885	0.05123	0.03837	0.10634	0.01244	0.03555	0.04484	0.08155	0.23409
3	0.54923	0.14077	0.26985	0.22486	0.43833	0.10809	0.23351	0.25673	0.39002	0.58884
4	0.8038	0.43765	0.56651	0.5087	0.73634	0.32643	0.521	0.55266	0.70454	0.84235
5	0.93175	0.74022	0.81216	0.75886	0.91339	0.62232	0.74954	0.78645	0.88054	0.94742
6	0.97493	0.91236	0.93034	0.89865	0.97563	0.84941	0.8771	0.9114	0.94844	0.98101
7	0.99135	0.9745	0.97146	0.95921	0.99402	0.94703	0.93883	0.96356	0.97454	0.99142
8	0.99812	0.99282	0.98822	0.98412	0.9987	0.98062	0.97015	0.98524	0.98555	0.99467
9	0.99919	0.99757	0.99505	0.99298	0.99972	0.99051	0.98457	0.99348	0.98934	0.9963
10	0.99953	0.9993	0.9965	0.99614	1	0.99472	0.9921	0.99669	0.99095	0.99787
	RAVEN for Test Context Only									
	CPM_large	gpt_ep50	gpt3_base	gpt3_finetune	pangu_a	rnn	smallt5-95	t5	unilm	zhouwenwang
1	0.48865	0.39468	0.24702	0.26906	0.79804	0.39433	0.27102	0.30358	0.48753	0.5979
2	0.84882	0.84342	0.5576	0.64379	0.99026	0.86825	0.67312	0.71238	0.8462	0.93149
3	0.93186	0.95315	0.69146	0.78834	0.99864	0.97316	0.82075	0.8623	0.94178	0.98074
4	0.96054	0.982	0.75251	0.85403	0.99979	0.99426	0.88017	0.92146	0.97059	0.9915
5	0.97461	0.99332	0.78886	0.88925	0.99993	0.99867	0.91524	0.95231	0.98308	0.99537
6	0.98259	0.99746	0.80871	0.90911	1	0.99957	0.93901	0.96997	0.98891	0.9971
7	0.98898	0.99876	0.82275	0.92242	1	1	0.95683	0.98105	0.99337	0.99826
8	0.99178	0.9994	0.83464	0.93158	1	1	0.97015	0.98684	0.99473	0.9988
9	0.99333	0.99968	0.84449	0.93612	1	1	0.98084	0.99066	0.99594	0.99915
10	0.9944	0.99982	0.85047	0.9387	1	1	0.98774	0.99315	0.99704	0.99924


==> sub/case_study.tex <==
\section{Examples of generated scripts}
\label{sec:appendix}

We present some generated crosstalk scripts as shown in Tab. \ref{tab:seq2seq},\ref{tab:gpt},\ref{tab:unilm}, and \ref{tab:gpt3}. The top 10 lines are the given raw scripts and the the following 10 lines are the generated ones.


\begin{table}[]
    \centering
    \scriptsize
    \begin{tabular}{ll}
    \toprule
    甲:相声演员李伟建。 \\
    乙:刘洪沂。\\
    甲:今天呢我们给您说段相声。 \\
    乙:刘老师。 \\
    甲:啊。 \\
    乙:先问问您。 \\
    甲:啊。 \\
    乙:中国这么多传统的节日，您最爱过哪个节啊? \\
    甲:爱过哪个节? \\
    乙:啊。\\
    \hline \\
    甲:我最爱过的是那个……  \\
    乙:您这么羞涩干嘛呀。  \\
    甲:那我最爱过的是春节。  \\
    乙:春节。  \\
    甲:啊。  \\
    乙:为什么呀?  \\
    甲:你想啊，新年伊始，万象更新，中国的传统节日大伙都这么过嘛。  \\ 
    乙:您今年多大岁数?  \\
    甲:我今年六十五岁。  \\ 
    乙:难怪。  \\
\bottomrule
    \end{tabular}
    \caption{The raw script}
    \label{tab:raw}
\end{table}

\begin{table}[]
    \centering
    \scriptsize
    \begin{tabular}{ll}
    \toprule
    甲:相声演员李伟建。 \\
    乙:刘洪沂。 \\
    甲:今天呢我们给您说段相声。 \\
    乙:刘老师。 \\
    甲:啊。 \\
    乙:先问问您。 \\
    甲:啊。 \\
    乙:中国这么多传统的节日，您最爱过哪个节啊? \\
    甲:爱过哪个节? \\
    乙:啊。 \\
    \hline
    甲:喜欢听节日。  \\ 
    乙:对。  \\
    甲:喜欢相声。  \\
    乙:喜欢。  \\
    甲:喜欢健美。  \\
    乙:喜欢。  \\
    甲:喜欢看。  \\
    乙:喜欢看。  \\
    甲:喜欢看。  \\
    乙:喜欢看。  \\
\bottomrule
    \end{tabular}
    \caption{The generated script from Seq2Seq}
    \label{tab:seq2seq}
\end{table}


\begin{table}[]
    \centering
    \scriptsize
    \begin{tabular}{ll}
    \toprule
    甲:相声演员李伟建。 \\
    乙:刘洪沂。 \\
    甲:今天呢我们给您说段相声。 \\
    乙:刘老师。 \\
    甲:啊。 \\
    乙:先问问您。 \\
    甲:啊。 \\
    乙:中国这么多传统的节日，您最爱过哪个节啊? \\
    甲:爱过哪个节? \\
    乙:啊。 \\
    \hline
    甲:寒食节。 \\
    乙:对呀。 \\
    甲:中国有句话叫"吃粽子怕死"。 \\
    乙:哦。 \\
    甲:而且呢也要过。 \\
    乙:是啊。 \\
    甲:尤其是端午节。 \\
    乙:诶。 \\
    甲:吃粽子。 \\
    乙:吃粽子怕死? \\
\bottomrule
    \end{tabular}
    \caption{The generated script from UniLM}
    \label{tab:unilm}
\end{table}


\begin{table}[]
    \centering
    \scriptsize
    \begin{tabular}{ll}
    \toprule
    甲:相声演员李伟建。\\
    乙:刘洪沂。\\
    甲:今天呢我们给您说段相声。\\
    乙:刘老师。\\
    甲:啊。\\
    乙:先问问您。\\
    甲:啊。\\
    乙:中国这么多传统的节日，您最爱过哪个节啊?\\
    甲:爱过哪个节?\\
    乙:啊。\\
    \hline
    甲:爱过传统节日。\\
    乙:这回你打算表演什么节目?\\
    甲:我找一下好节目啊，让您开眼。\\
    乙:等会儿。\\
    甲:民主席是谁啊?\\
    乙:哈利波特。\\
    甲:好啊。\\
    乙:他在美国还给安排了。\\
    甲:怎么没有选项啊?\\
    乙:你们也去呗!\\
\bottomrule
    \end{tabular}
    \caption{The generated script from GPT}
    \label{tab:gpt}
\end{table}


\begin{table}[]
    \centering
    \scriptsize
    \begin{tabular}{ll}
    \toprule
    甲:相声演员李伟建。\\
    乙:刘洪沂。\\
    甲:今天呢我们给您说段相声。\\
    乙:刘老师。\\
    甲:啊。\\
    乙:先问问您。\\
    甲:啊。\\
    乙:中国这么多传统的节日，您最爱过哪个节啊?\\
    甲:爱过哪个节?\\
    乙:啊。\\
    \hline
    甲:嗯。\\
    乙:啊。\\
    甲:爱过哪个节?\\
    乙:啊。\\
    甲:我觉得，爱过的节日，是农历新年。\\
    乙:哦。\\
    甲:因为我们中国人，最重要的一个节日，就是农历新年。\\
    乙:那么您呢，您最爱过的一个人呢?\\
    甲:我最爱过的一个人?\\
    乙:啊。\\
\bottomrule
    \end{tabular}
    \caption{The generated script from GPT3}
    \label{tab:gpt3}
\end{table}

% \begin{table*}[t]
% \centering
% \scriptsize
% % \resizebox{\linewidth}{!}{
% \begin{tabular}{llll}
% \hline
% & Case 1: translation example that needs context                        &  & Case 2: translation example that do not need context                                                                                              \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Previous \\ sentences\end{tabular}} & 我第一次在一个饭店中吃到这种鱼,位置在西班牙南部。                                            &  & \multirow{2}{*}{到了1982 年，一家具有环保意识的西班牙公司购买了这块地。}                                                                                                   \\
% & I first ate it at a restaurant in southern Spain.                     &  &             \\
% & 很久以前一个记者朋友和我说过这里。                                                    &  & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}And so in 1982, a Spanish company with an environmental conscience \\ purchased the land. \end{tabular}} \\
% & A journalist friend had been talking about this fish for a long time. &  &    \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Current \\ sentences\end{tabular}}  & 她可以说是个\textbf{媒人}                                        &  & 他们做过什么？  \\
%  & She kind of set us up.                                                &  & What did they do?  \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Later \\ sentences\end{tabular}}    & 那条鱼在桌子上很亮, 有着光晕，白色的那种。                                               &  & 他们逆转了水流的方向。\\
% & It came to the table a bright, almost shimmering, white color.        &  & They reversed the flow of water. \\ \hline
% \end{tabular}
% \caption{\label{tab:cases}a translated Xiangsheng scripts. }
% % }
% \end{table*}






==> sub/human-evaluation.tex <==
\begin{table}[]
    \centering
    \small
    \begin{tabular}{llll}
    \toprule
    \textbf{Models} & \textbf{Type} &   \textbf{Satisfaction}  & \textbf{Ranking}  \\
    \midrule
        Raw  & - & 89.14\% & 4.44 \\
        Seq2seq & train from scratch & 16.14\% &  2.05 \\
        GPT  &  pre- and fine-tuning & 30.57\% &  2.52 \\
        GPT-3 & pre-training & 45.14\% & 2.95 \\
        UniLM &  pre- and fine-tuning &  46.14\% &  3.03 \\
    \bottomrule
    \end{tabular}
    \caption{Human assessment for crosstalk generation}
    \label{tab:human}
\end{table}

Based on the human assessment,  we define 1) `satisfaction'  as the average satisfaction score among these 50 scripts; 2)`ranking score' as the average ranking score. As shown in Table \ref{tab:human}, raw scripts achieve the best satisfaction since it is manually created by humans. Seq2seq performs the worst. This may be due to Seq2seq does not utilize the pre-training. Among these pre-trained models, UniLM outperforms others (including Seq2seq, GPT, GPT-3). Note that both GPT and UniLM fine-tuning on the train set while GPT-3 does not -- the generation of GPT-3 is zero-shot and the training dataset of $C^3$ is invisible for it). We should notice that GPT-3 is mainly for English, but its generation in Chinese is pretty good and sometimes exceptional. There are 14 participants evaluated on 50 scripts. The Fleiss' kappa among these participants is 0.366.



\benyou{RAVEN}

\paragraph{Conclusion} Based on the human assessment, we could preliminarily conclude that \textit{the best generation approach achieves pretty good crosstalk with nearly 50\% satisfaction, but it is highly worse than raw scripts with the satisfaction of 89\%.} \benyou{update}

The reason could be twofold as below.
\textbf{First, evaluation criterion for humor generation is not satisfied}: it lacks an evaluation criterion that could evaluate humor generation. Observing the inconsistency between Tab. \ref{table:overall_result} and Tab. \ref{tab:human}, a better performance evaluated using BLEU2 and BLEU4 does not lead to a better performance in human assessment, this probably suggest that BELU or related metrics for generation is not inappropriate for humor generation.  Text-based evaluation criterion for humor generation may not make sense since humor itself is diverse and subjective that does not have textual ground truth. 
While human assessment is expensive and cannot gives real-time feedback during model training. A better evaluation criterion for humor is expected.
\textbf{Secondly, dataset scale is relatively-small}: The dataset in $C^3$ has nearly 10,000 dialogue, which is relatively large in the humor generation dataset. However, it may be far away for natural language generation models like GPT. In this matter, super large-scaled pre-trained models like GPT-3 may help.
% but unfortunately, GPT-3 is currently not very friendly to generation in Chinese.



% we observed that GPT performs well to complate a text with a regular pattern like an integrative dialogue with  peng and dou. 

% treat previous utterance as the the few shots for following utterance.

% Few-shot Generation using GPT-3

% Since we do not check with  pre-trained language models with various-scaled size. the reported numbers do not admit that which model is better than other, but to  show some intuitive performance with existing accessible models.



==> sub/new_case.tex <==
\section{Generated Xiangsheng script examples}
\label{sec:examples}
We randomly select some generated Xiangsheng script examples as below.



 
 \begin{table*}[] 
   \centering 
   \scriptsize 
    \begin{tabular}{p{0.25cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}} 
    \toprule 
    &Raw & RNN & Unilm & GPT & GPT 3 \\  
   \midrule
甲&\multicolumn{5}{p{16cm}}{他让你再来一个，刚才，啊，你也辛苦了，今天二，好，再切一个，好。}\\
乙&\multicolumn{5}{p{16cm}}{你跑这谈恋爱了是吧!}\\
甲&\multicolumn{5}{p{16cm}}{今天呢是我们暑期的第一场。}\\
乙&\multicolumn{5}{p{16cm}}{哎。}\\
甲&\multicolumn{5}{p{16cm}}{刚才呢张文甫先生。}\\
乙&\multicolumn{5}{p{16cm}}{对。}\\
甲&\multicolumn{5}{p{16cm}}{~文工团曲艺队的队长。}\\
乙&\multicolumn{5}{p{16cm}}{嗯。}\\
甲&\multicolumn{5}{p{16cm}}{在中国这个快板界，包括我们创作都是相当的了不得。}\\
乙&\multicolumn{5}{p{16cm}}{创作表演都是一流。}\\
\midrule
甲&高凤山先生的高足。&这个时候就是一段时间。&哎。&那不假。&嗯，他们现在还在江苏巡回演出呢。\\ \hline
乙&对。&嗯。&尤其像那些快板大家伙儿都喜欢看的节目。&时代在发展，人们更加的快节奏全都变了。&哦。\\ \hline
甲&懂快板的朋友们都知道。&刚才咱们学校的艺术家。&啊!&比如说您看刚才那个快板书，叫《数来宝》。&他们还是全国第一名的呢。\\ \hline
乙&啊。&哎。&比如说《新春打靶》、《武松打靶》、&这个节目是四段。&哦。\\ \hline
甲&曲艺里边有一句话，学会王高李有个好身体，这其中这高，就是高凤山先生。&前几天早晨起来，他们也没听清楚。&等会儿等会儿吧你等会儿吧你等会儿吧你等会儿吧你等会儿吧你等会儿吧&讲究是四段儿。&~文工团曲艺队的队长张文甫先生。\\ \hline
乙&对。&对。&怎么了&讲究是这四段儿。&嗯，刚才，你说，我们的舞台包括表演都是一流。\\ \hline
甲&本来我们这叫师叔。&后来我们班长的特别高兴。&就咱们这种形式表达出来的内容太少了。&哪四段儿?&创作表演都是一流。\\ \hline
乙&对。&哦。&哦。&“元”，表示什么?&创作表演都是一流，你说我们的舞台包括表演都是一流，你说这个是不是很有意思?\\ \hline
甲&我说您使一段传统的节目就行。&一般的形式都是为了节目。&但是也有人爱听。&“元”，表示春天。&嗯，很有意思!\\ \hline
乙&嗯。&嗯。&哦。&噢，明白了。&哎呀!好了!好了!好了!好了!好了!好了!好了!好了!好了!(观众给节目打手势) 《时代》杂志上看到这个舞台就想要采访我们, 因为这个舞台\\ 
\bottomrule 
   \end{tabular} 
    \caption{The raw script and generated scripts 2} 
    \label{tab:raw2} 
 \end{table*}




\begin{table*}[] 
   \centering 
   \scriptsize 
    \begin{tabular}{p{0.25cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}} 
    \toprule 
    &Raw & RNN & Unilm & GPT & GPT 3 \\  
   \midrule
甲&\multicolumn{5}{p{16cm}}{亲爱的观众朋友们，大家……}\\
乙&\multicolumn{5}{p{16cm}}{非常高兴，北京电视台的舞台，我们非常地熟悉了。}\\
甲&\multicolumn{5}{p{16cm}}{对对对。}\\
乙&\multicolumn{5}{p{16cm}}{您看这一年一年过得真快。点点如潮，笔笔如刀，是刀刀催人老。}\\
甲&\multicolumn{5}{p{16cm}}{您这都什么词啊这都是。}\\
乙&\multicolumn{5}{p{16cm}}{一句好词啊，时间过得太快了。}\\
甲&\multicolumn{5}{p{16cm}}{那倒是。}\\
乙&\multicolumn{5}{p{16cm}}{我这边这位王声老师，大家都非常的熟悉。}\\
甲&\multicolumn{5}{p{16cm}}{认识我。}\\
乙&\multicolumn{5}{p{16cm}}{满腹经纶。}\\
\midrule
甲&别捧我，别捧我。&哎。&是。&谁呀。&满腹经纶。\\ \hline
乙&这么一个特别好的相声演员，，除了这个狗齿伶，口齿伶俐之外呢，知识也特别的丰富。一直说人家学文学，文学、历史这是王声老师身上的两大法宝。&你看咱们这个节目，有一个问题。&四门功课说学逗唱。&最人知的就是说你，见了面头郭德纲，先生于2014年7月份认识我大爷啊继续在新长58年了。&今天这个节目，我们邀请了一位特别的嘉宾，来到这里。\\ \hline
甲&不，也就是看过两本书。&什么问题呀。&没错。&哎呦喂，你停一下行不行啊?什么叫给大伙儿讲来着。&来到这里。\\ \hline
乙&不是两本书，天天在那儿翻纸，铺嚓铺嚓。这不到猴年了嘛，今天当着所有咱们观众朋友的面，也是过年了。&您想听吗?&最拿手的就数他。&爱听相声嘛，每个人得多知事。&一位非常的有名的人士，是曾经在北京电视台工作的，在北京电视台工作的时候，是一位非常好的主持人。\\ \hline
甲&对。&怎么着?&嗯。&知道事情?&他现在是一位很有名气的文学家。\\ \hline
乙&考一考你。&我知道为什么要求爱好者。&在北京曲艺团校园里边，能够走到国内外。&这句话是有理。&很有名气。\\ \hline
甲&你说在历史的长河当中啊，这个历史的长河当中。&您别激动。&很少见面。&怎么讲呢?&我们非常的熟悉他，就是……\\ \hline
乙&您等会儿，您等会儿。您刚才是电打着你了，是怎么这一下。&我觉得这个节目中暑假期，可以提醒。&因为什么呢?&不要光知道事情啊!&王声老师。\\ \hline
甲&没，没有。&您这是干嘛呀?&因为我们哥两是传道接代的好朋友。&还当校长呢!&王声老师。王声老师来到这里，就是要和我们聊一个问题。王声老师：大家好！我是王声老师。我想问大家一个问题：“如果你看到了一个不说话的人，你会怎么想呢?\\ 
\bottomrule 
   \end{tabular} 
    \caption{The raw script and generated scripts 3} 
    \label{tab:raw3} 
 \end{table*}




\begin{table*}[] 
   \centering 
   \scriptsize 
    \begin{tabular}{p{0.25cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}} 
    \toprule 
    &Raw & RNN & Unilm & GPT & GPT 3 \\  
   \midrule
甲&\multicolumn{5}{p{16cm}}{弟弟你想起来了?}\\
乙&\multicolumn{5}{p{16cm}}{想起什么来了?这不海尔兄弟嘛。}\\
甲&\multicolumn{5}{p{16cm}}{对，我们就是海尔兄弟呀。}\\
乙&\multicolumn{5}{p{16cm}}{我们是海尔兄弟?}\\
甲&\multicolumn{5}{p{16cm}}{嗯。}\\
乙&\multicolumn{5}{p{16cm}}{我们穿的有点多了吧?}\\
甲&\multicolumn{5}{p{16cm}}{长大了要懂得羞耻。}\\
乙&\multicolumn{5}{p{16cm}}{废话，你得知道羞耻了，还海尔兄弟了。你见过穿裤衩，站这说相声的吗?}\\
甲&\multicolumn{5}{p{16cm}}{小时候就可以呀，小时候多好啊。小小少年，没有烦恼，穿着裤衩，到处跑。}\\
乙&\multicolumn{5}{p{16cm}}{俩臭流氓，你听听。}\\
\midrule
甲&当然现在不让穿了。&你这是什么意思?&你看，我们小时候穿的多好啊。&但是我什么也没有见过。&哼，你也不比我好。\\ \hline
乙&废话。&我想当初一个演员，有点击率。&是吗?&您说，咱们有这个吗?&这是谁说的?\\ \hline
甲&我俩都三十多了，往这一站说相声。&什么叫吐槽?&哎呀，小时候穿裤衩，到处跑。&您的意思是?&我说的啊。\\ \hline
乙&表演。&报告长。&俩臭流氓。&我……&你个臭流氓，你不要瞎说。\\ \hline
甲&当然这算好的。&你知道吗?&哎哟呵，真不错。&你可拉倒吧。&我说的是真的。\\ \hline
乙&这就算好了?&知道。&怎么样?&没有。&那你是怎么知道的?\\ \hline
甲&当年，跟我们在电视台，一块录动画片那些小伙伴，现在好多都不干这行了。&你别说了，这句话太难过了。&跟大伙儿分享一点笑话。&你可拉倒吧，我都不知道了。&因为我就是海尔兄弟呀。\\ \hline
乙&唉，你先等会，你先等会，咱还有小伙伴。&谁说的?&好啊。&嗨，就他长得这么丑。小时候呢?&那你是怎么知道的?\\ \hline
甲&小伙伴你也不记得了?&你觉得裸睡怎么样?&其实我觉得，穿裤衩，很难。&就我现在实力早晚会好吧。上一出去喝点儿酒抽烟，上网、看节目去睡觉，娱乐购物点心思开放，要坐车时间打几圈游戏玩些地方戏?&因为我就是海尔兄弟呀。\\ 
\bottomrule 
   \end{tabular} 
    \caption{The raw script and generated scripts 4} 
    \label{tab:raw4} 
 \end{table*}




\begin{table*}[] 
   \centering 
   \scriptsize 
    \begin{tabular}{p{0.25cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}} 
    \toprule 
    &Raw & RNN & Unilm & GPT & GPT 3 \\  
   \midrule
甲&\multicolumn{5}{p{16cm}}{您给我个机会让我也来一回行不行。}\\
乙&\multicolumn{5}{p{16cm}}{你想再学习一下。}\\
甲&\multicolumn{5}{p{16cm}}{我演你那角色呀。}\\
乙&\multicolumn{5}{p{16cm}}{那这样吧角色互换，你呢来这个小男孩我来这个小女孩。}\\
甲&\multicolumn{5}{p{16cm}}{可以呀。}\\
乙&\multicolumn{5}{p{16cm}}{咱俩就是体验一下。}\\
甲&\multicolumn{5}{p{16cm}}{行行行。}\\
乙&\multicolumn{5}{p{16cm}}{你来这边。}\\
甲&\multicolumn{5}{p{16cm}}{行行行我体验一下。}\\
乙&\multicolumn{5}{p{16cm}}{这样行吧你呢就按我刚才那套词。}\\
\midrule
甲&你那套词。&我这个词都没有。&怎么了。&我说一大套词。&好。\\ \hline
乙&一模一样的来。&行了行了，你别介绍我来吧。&来一个小男孩。&可以呀。&每句话你都要给我响铃。\\ \hline
甲&小姐姐你撞到我了。&(学长江尾)&可以呀。&你来这个小女孩。&好。\\ \hline
乙&对不起我撞到你哪儿了。&哎呀，我这会儿太大了。&咱俩就是体验一下。&行。&这样行吧，你先来。\\ \hline
甲&你撞到我哪儿了，哦你就撞我这儿了。&怎么着?&行行行。&可以，你先来。&我是小男孩，我叫林林。\\ \hline
乙&我撞你这儿咋啦。&我这胳膊长短腿，膀大腰圆。&你看现在有人给你介绍一个比较合适的。&我看您来一回。&这么多年了，林林在哪里呢？\\ \hline
甲&你撞我这就不行。&我这眼睛乖。&谁呀。&我再来一回。&我去了趟公园，去了趟公园。\\ \hline
乙&不行我就撞了。&(冲竹板)&裘英俊。&咱们两个人。&啊！什么时候去的呀？\\ \hline
甲&你还真跟着来劲你。&(惊)嘿，这位干嘛呀。&裘英俊。&站在街上正合适。&我上个星期去的。\\ \hline
乙&哎呀你这玩命来了你，我刚才是这样吗。&(指乙)&你看像吗。&行。&啊！上个星期去的呀！你怎么还不回来呢？\\ 
\bottomrule 
   \end{tabular} 
    \caption{The raw script and generated scripts 5} 
    \label{tab:raw5} 
 \end{table*}




\begin{table*}[] 
   \centering 
   \scriptsize 
    \begin{tabular}{p{0.25cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}} 
    \toprule 
    &Raw & RNN & Unilm & GPT & GPT 3 \\  
   \midrule
甲&\multicolumn{5}{p{16cm}}{好，就算不是世界各地的，那也是这么多热心观众来到这儿了。}\\
乙&\multicolumn{5}{p{16cm}}{那倒是。}\\
甲&\multicolumn{5}{p{16cm}}{而且我觉得大伙儿来到这儿，只有一个目的。}\\
乙&\multicolumn{5}{p{16cm}}{什么目的?}\\
甲&\multicolumn{5}{p{16cm}}{就看你来了。}\\
乙&\multicolumn{5}{p{16cm}}{(笑)}\\
甲&\multicolumn{5}{p{16cm}}{这演员特别好。}\\
乙&\multicolumn{5}{p{16cm}}{不行。}\\
甲&\multicolumn{5}{p{16cm}}{招人喜欢。}\\
乙&\multicolumn{5}{p{16cm}}{没有没有。}\\
\midrule
甲&每场演出都兢兢业业，一丝不苟的在台上装弱智。&没有。&不是，你这个演员怎么就招人喜欢了?&不用骄傲的表演。&我们认为他很棒。\\ \hline
乙&应该的。&不会说话。&我们俩一直在研究。&是，咱别争了。&这可不是一般的演员。\\ \hline
甲&这样的演员我很佩服。&那怎么办呢?&研究什么呢?&咱得看事啊!&就是那种你不知道他在做什么，但是你觉得很有意思。\\ \hline
乙&你别佩服，不用佩服我，我在台上装弱智你就佩服我呀?我们演员我们台上塑造什么人物形象，就是演出需要。&因为我们在座的各位观众朋友们，他们都愿意给我们表演一段相声。&这个演员的基本特征。&我跟你看就不能低调点。&那也是一种演员。\\ \hline
甲&你们演员啊，我是说你们这个行业。&对。&啊!&应该的。&我想这种演员就像一个魔术师，你看到了，却不知道他在干啥。\\ \hline
乙&怎么着?&我们两个人往台上一站，其实现在已经开始了。&他们得像个男孩子似的。&因为我本身对待艺人才啊?&(笑)\\ \hline
甲&既神秘又特殊。&嗯。&哎呦喂。&我这个人啊长得高级、优秀、优雅，而且淡泊名利。&这样的人我喜欢。\\ \hline
乙&也不能这么说。&我们这个场合社会主题特别的热情。&怎么回事?&您等会儿，您说那是什么呀?&(笑)\\ \hline
甲&你看像我们这种普通行业，跟你根本比不了。&是。&你瞧，这男孩子多可爱呐。&高级、干派?&(英文)He is a very interesting actor. He is very good.  (中文)那个人特别好看，特别好演。\\ \hline
乙&咱们都一样。&我们三个人能够站在这儿，第二次以后再来一回。&废话，谁可爱呀?&学员啊。&(英文)He is a good actor. He is so funny.  (中文)他很好看，很好玩。\\ 
\bottomrule 
   \end{tabular} 
    \caption{The raw script and generated scripts 6} 
    \label{tab:raw6} 
 \end{table*}




\begin{table*}[] 
   \centering 
   \scriptsize 
    \begin{tabular}{p{0.25cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}} 
    \toprule 
    &Raw & RNN & Unilm & GPT & GPT 3 \\  
   \midrule
甲&\multicolumn{5}{p{16cm}}{好嘛，这俩人调个儿啦。}\\
乙&\multicolumn{5}{p{16cm}}{同学们对“二儿”都很惋惜。}\\
甲&\multicolumn{5}{p{16cm}}{这回你该说说晓霞了、}\\
乙&\multicolumn{5}{p{16cm}}{行，晓霞旁边同学忘没忘?}\\
甲&\multicolumn{5}{p{16cm}}{不是，你说的那是“二儿”呀。}\\
乙&\multicolumn{5}{p{16cm}}{晓霞左旁边的，我说是右旁边那个。}\\
甲&\multicolumn{5}{p{16cm}}{我不记得。}\\
乙&\multicolumn{5}{p{16cm}}{小石头，}\\
甲&\multicolumn{5}{p{16cm}}{小石头?}\\
乙&\multicolumn{5}{p{16cm}}{画画画得特别好。}\\
\midrule
甲&还给晓霞画过像。&“东边”。&晓霞，你说的那是…二儿…呀?&这么说那也是不好画，整个德云花的。&是啊，小石头的画很好。\\ \hline
乙&他的画在全国获过奖。&“山东人”。&对、对!&对。&小石头，你们认识吗?\\ \hline
甲&最大的理想是当齐白石。&“山东人海”。&晓霞把笔拿过来了:"小石头，画得特别好，大家伙鼓掌欢迎他给我写一&特别是看起来的画切碎了，可以找一个人拍照留作纪念吧。&我们都是同学。\\ \hline
乙&就这小石头。&“昔日月”。&呵!&啊!&哦，那你们比较熟悉些?\\ \hline
甲&啊?&“昔月如霜”。&噢，又改啦!&这里面都是你们家的?&嗯，我们都是同一个班的。\\ \hline
乙&接他妈妈的班给清洁队扫大街呢。&“嗯”。&她用笔在桌子上照着我，我就看见了。&我们家的。&那你们认识多久了?\\ \hline
甲&这照理想比差着远了点也。&“若先生”。&嗯，这个老师很幽默。&去，一谁呀?&一年多了。\\ \hline
乙&小石头不这么认为，前些日子参加电视台演讲比赛还说这件事呢。&“哎，兄弟姐妹们，你还别说，今儿咱们再来一个。”&晓霞把纸条递过去了:"谢谢老师，谢谢老师，我想起来了，我要写一张&我们家的!&那你们当时在哪里认识的?\\ \hline
甲&啊?&“好嘞!”&咳!&去，小石头。&小石头在学校里认识的。\\ \hline
乙&演讲的好，动作设计的有意思。&“哎，这个意思是吗?”&她还嘱咐我:"先生，请您注意安全，千万不能乱扔东西，否则会伤及您&小石头?&小石头，你怎么会在学校里认识的?\\ 
\bottomrule 
   \end{tabular} 
    \caption{The raw script and generated scripts 7} 
    \label{tab:raw7} 
 \end{table*}




\begin{table*}[] 
   \centering 
   \scriptsize 
    \begin{tabular}{p{0.25cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}} 
    \toprule 
    &Raw & RNN & Unilm & GPT & GPT 3 \\  
   \midrule
甲&\multicolumn{5}{p{16cm}}{我们首先看一下，其他剧场相声的报价。}\\
乙&\multicolumn{5}{p{16cm}}{那我们来听一听。}\\
甲&\multicolumn{5}{p{16cm}}{国家大剧院一千五百块，农业展览馆二千块，北京动物园五千块。}\\
乙&\multicolumn{5}{p{16cm}}{跟猴儿一块说相声啊?}\\
甲&\multicolumn{5}{p{16cm}}{那么我们今天的相声卖多少钱呢?}\\
乙&\multicolumn{5}{p{16cm}}{卖多少钱哪?}\\
甲&\multicolumn{5}{p{16cm}}{八毛钱，比其他剧场足足便宜了三百块呀!}\\
乙&\multicolumn{5}{p{16cm}}{这都什么账头啊这是?}\\
甲&\multicolumn{5}{p{16cm}}{赶快拨打我们的销售热线，二百五加三八加十三点加二。}\\
乙&\multicolumn{5}{p{16cm}}{全是傻数啊。}\\
\midrule
甲&你还在等什么?我们的相声真的是非常非常便宜，非常非常省钱，非常非常物超所值，非常，非，非，灰化肥发挥会发挥，灰化肥挥发会挥发，灰化肥发灰，黑化肥发黑，你来来这个。&这是一百块钱。&好，接下来的节目我们就卖了。&还不是为了保证顾客能够接受我们的锻炼?说半天连狗口吐白沫都没有。&你拨了?\\ \hline
乙&我还真来不了这个，不是，说这么热闹你是干什么的呀?&不少!&等会儿吧，你怎么还卖呀?&嗨!这么跟你说吧，我们的宣传语言太烂了。&拨了啊。\\ \hline
甲&我是春节大卖场的促销专家。&老百姓都知道，中国三百多人在哪儿上?&不卖也得卖呀!&那你怎么说的呀?&你说什么?\\ \hline
乙&你还是专家。&没有。&为什么呀?&我们的宣传语言很烂，说出来谁敢听呀?&我说，我是一个人，一个人来。\\ \hline
甲&提起我来，全世界都闻名。&为什么呢?&你想啊，相声它是说、学、逗、唱，讲究四门基本功课，你知道吗?&你们的宣传语是什么?&这么小的数目，我们还是先报给你吧。\\ \hline
乙&您叫?&因为他们也没有资金。&当然知道了。&语言，什么味儿?&好啊。\\ \hline
甲&迈克尔杰克逊。&啊?&你问谁呀?&发情达理想，全身有力;只要思想纯真，事业自己解放心不下去批评，斤斤计较。我们坚决反对!&一共十五块钱，您有现金吗?\\ \hline
乙&你叫什么?李伟健:不不，卖货了接过去。&当然有一种花钱的。&问我呀。&怎么个意思?&有呀!您给我十五块钱。\\ \hline
甲&卖货了接过去。&有什么?&哦，你问我，你问我，你能回答吗?&你比方说，我们的宣传语言太烂，容易产生歧义。&不用给十五块钱了，跟我来吧!\\ \hline
乙&说快了，迈克尔杰克逊。武宾:你都卖什么呀?&花钱的价值。&当然能了。&通过我们的革命广告语言，使人印象丰富。&走呀!来了呀!(打出门)大伙儿都来了呀!大伙儿都来了呀!大伙儿都来了呀!大伙儿都来了呀!(打出门)大伙儿都来了呀!大伙儿都来了呀!大伙儿都来了呀!大伙儿都来了呀!(打出门)大伙儿都来了呀!大伙儿都来了呀!大伙儿都来了\\ 
\bottomrule 
   \end{tabular} 
    \caption{The raw script and generated scripts 8} 
    \label{tab:raw8} 
 \end{table*}




\begin{table*}[] 
   \centering 
   \scriptsize 
    \begin{tabular}{p{0.25cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}} 
    \toprule 
    &Raw & RNN & Unilm & GPT & GPT 3 \\  
   \midrule
甲&\multicolumn{5}{p{16cm}}{谢谢。}\\
乙&\multicolumn{5}{p{16cm}}{哎。}\\
甲&\multicolumn{5}{p{16cm}}{感谢大伙儿热烈的掌声。}\\
乙&\multicolumn{5}{p{16cm}}{谢谢大家。}\\
甲&\multicolumn{5}{p{16cm}}{哎都说你们相声演员的这个眼光特别的独到。}\\
乙&\multicolumn{5}{p{16cm}}{有这么说的。}\\
甲&\multicolumn{5}{p{16cm}}{甭管什么人只要打您眼前这么一过，您不用拿正眼瞧人家。}\\
乙&\multicolumn{5}{p{16cm}}{对。}\\
甲&\multicolumn{5}{p{16cm}}{拿这个旁光这么一扫大概。}\\
乙&\multicolumn{5}{p{16cm}}{您等会儿您等会儿，没听说过，好不来个人我不拿正眼瞧他。}\\
\midrule
甲&对呀。&我这是逗哏的。&你看。&去!&对。\\ \hline
乙&我拿膀胱一扫。&我说你别捯气，他也得跟您搭档。&他就是一个人的眼光特别独到。&你怎么还正眼看人家?&您等会儿您等会儿，没听说过，好不来个人我不拿正眼瞧他。\\ \hline
甲&有问题吗这玩意儿。&嗯。&嗯。&别说了，什么叫正眼圆呢?我这一直是右手先生吗。&对。\\ \hline
乙&你不嫌骚气吗。&尤其是这个捧哏的，我特别喜欢看相声。&有什么区分吗?&左边那个反光镜啊?&这样的话，那么大家都是相声演员，大家都是相声演员，大家都是相声演员，大家都是相声演员，大家都是相声演员。\\ \hline
甲&这什么词。&嗯。&当然有区别啦。&我用手比划右边的，算术您也不懂。&哎。\\ \hline
乙&什么叫膀胱一扫啊。&我觉得太棒了，比如说，这位大伙儿都知道。&都有区别。&我算术上成功还可以，&那么我们就先说一个词。\\ \hline
甲&旁光不明白吗。&嗯。&哎。&瞧见了嘛。&哎。\\ \hline
乙&谁不懂啊。&但是我想起来了，因为这个舞台上表演艺术家，当然值钱多了。&您像刚才那段相声演员叫王宝强。&这把我就震撼了。&让我们先说一个词。\\ \hline
甲&给你解释解释，上眼瞧啊。&对。&哦。&我一直在这儿就哆嗦哪。&哎。\\ \hline
乙&怎么的。&拿手机给我举个例子。&王老师非常优秀。&紧张什么呀?&让我们先说一个词。\\ 
\bottomrule 
   \end{tabular} 
    \caption{The raw script and generated scripts 9} 
    \label{tab:raw9} 
 \end{table*}




\begin{table*}[] 
   \centering 
   \scriptsize 
    \begin{tabular}{p{0.25cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}} 
    \toprule 
    &Raw & RNN & Unilm & GPT & GPT 3 \\  
   \midrule
甲&\multicolumn{5}{p{16cm}}{亲爱的观众朋友们。}\\
乙&\multicolumn{5}{p{16cm}}{非常开心。}\\
甲&\multicolumn{5}{p{16cm}}{啊。}\\
乙&\multicolumn{5}{p{16cm}}{也非常激动。}\\
甲&\multicolumn{5}{p{16cm}}{没错。}\\
乙&\multicolumn{5}{p{16cm}}{2019年。}\\
甲&\multicolumn{5}{p{16cm}}{对。}\\
乙&\multicolumn{5}{p{16cm}}{新中国成立七十周年。}\\
甲&\multicolumn{5}{p{16cm}}{整整七十年。}\\
乙&\multicolumn{5}{p{16cm}}{高老师。}\\
\midrule
甲&您说。&嗯。&啊。&嗯。&啊。\\ \hline
乙&咱们来个现场采访怎么样?&心里特别的激动。&为祖国建设贡献了很多东西。&今年已经五十多岁了。&非常激动。\\ \hline
甲&采访谁呢?&哎。&没错。&可不是嘛，您还活着呢。&是啊。\\ \hline
乙&采访您呢。&因为中国相声界的文明史。&但是今天高老师身体不太好。&活到六十一了。&我们这个时代的中国人。\\ \hline
甲&问问我?&对。&哦。&老人们还挺自豪。&是啊。\\ \hline
乙&对呀。&因为他们的艺术更多了。&特别需要锻炼。&开车上班去了。&在这个时代里面。\\ \hline
甲&问我什么呀?&怎么呢?&需要健身嘛。&嗯。&是啊。\\ \hline
乙&我来采访您。&经验。&每天早晨起来就练习。&给老人家了一个亲戚。&见证了中华民族的伟大复兴。\\ \hline
甲&您说说。&哦。&嗯。&特别开心，听相声首先要有一个好习惯。&是啊。\\ \hline
乙&您说我们今天这个生活，您幸福吗?&比如说郭德纲的徒弟。&然后再做瑜珈。&什么习惯?&所以我们要感谢祖国，感谢祖国对我们的养育，对我们的教育，对我们的爱护，对我们的保护，所以这一年，这一年，这一年……\\ 
\bottomrule 
   \end{tabular} 
    \caption{The raw script and generated scripts 10} 
    \label{tab:raw10} 
 \end{table*}




\begin{table*}[] 
   \centering 
   \scriptsize 
    \begin{tabular}{p{0.25cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}} 
    \toprule 
    &Raw & RNN & Unilm & GPT & GPT 3 \\  
   \midrule
甲&\multicolumn{5}{p{16cm}}{我也打，不行我电话没费了。}\\
乙&\multicolumn{5}{p{16cm}}{你没费，我打，喂，导演，我盛伟，咱不是评选那个优秀家风好演员嘛?我这个人我毛遂自荐，我认为我还是比较合适的，为什么?我家风好啊，我经常帮助那个，我们楼上的那个孤寡老人。}\\
甲&\multicolumn{5}{p{16cm}}{那是他姥姥。}\\
乙&\multicolumn{5}{p{16cm}}{对，她是我姥姥，她是我姥姥，她也是孤寡老人，为什么?因为我姥姥姓孤，叫孤寡。}\\
甲&\multicolumn{5}{p{16cm}}{蛤蟆。}\\
乙&\multicolumn{5}{p{16cm}}{你才蛤蟆呢，喂喂，导演，没说你，我是说我那个蛤蟆姥姥，我跟她，我就是给她打扫打扫卫生。}\\
甲&\multicolumn{5}{p{16cm}}{你行了，你给我拿过来吧你，导演，你还得听我说，我不是老王卖瓜自卖自夸，我这人品太好了，我这家风也好，你知道吗?我们初中老师退休，我给他办了六十多场感恩会。}\\
乙&\multicolumn{5}{p{16cm}}{他小学四年级之后就不上了。}\\
甲&\multicolumn{5}{p{16cm}}{不，不是四年级不上学了，他说我，他说我四年级个儿头就不上了您知道吗?所以说呀。}\\
乙&\multicolumn{5}{p{16cm}}{是真能编。}\\
\midrule
甲&还得是我上。&我是一个人，你看这样的话，就像您这么说。&我说你这个人，就是有点儿不对劲。&什么话呀，我们十六个人就是我的学生。&你给我拿过来，我跟你说，你们这个奖啊，这个奖的评选，我们小学老师也可以参加吗?\\ \hline
乙&我电话你说着，导演，还得选我。&怎么了?&谁说的?&啊，你们老师多大了?&不行，不行。\\ \hline
甲&他家风有问题。&我刚才那位老师可以给你介绍一下，我是大学生。&导演。&四年级。&为什么不行?\\ \hline
乙&我家风挺好，真的。&我是来自北京的学生。&你给大伙学一回。&我们老师本科毕业后谈的。&因为小学老师是最差的。\\ \hline
甲&他人品也不行他，你选他。&我是秦始皇的，我在哪儿呢?&我还真能编。&哎呦妈呀，那不是同一个。&那怎么会呢?我们小学老师是最好的啊。\\ \hline
乙&评选结果出来了，谁呀?李菁，不是，他，哦，李菁把补助那三千块钱捐给敬老院了，哦，行，再见，李菁把钱捐给敬老院了。&我是河北梆子。&你来来。&这什么时候宣传了?&是最差的。\\ \hline
甲&要这么说，人家李老师那叫实至名归。&您听着，我们这儿都演出了。&我现在是小孩子嘛。&这是90年代的事儿了，您听我说呀。&那怎么会呢?我们小学老师是最好的啊。\\ \hline
乙&我怎么感觉有点不好意思呢?&对。&嗯。&您这学术真没有白用。&因为小学老师贡献度太大了，所以说呀。\\ \hline
甲&咱这脸还是脸吗?&我是郭德纲，今天我们仨月饼啊，您想当初二十几块钱。&我告诉你，我现在特别聪明。&这都什么年代啦?&可是你看看，比如说高中的时候呢，比如说高中时候呢，我们数学老师走了一年之后，结果就觉得上不了数学了，全校都上不了数学了。\\ \hline
乙&是不是做错了?&三十元?&哦。&您说那时候干嘛的?&都上不了数学了。\\ 
\bottomrule 
   \end{tabular} 
    \caption{The raw script and generated scripts 11} 
    \label{tab:raw11} 
 \end{table*}




\begin{table*}[] 
   \centering 
   \scriptsize 
    \begin{tabular}{p{0.25cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}} 
    \toprule 
    &Raw & RNN & Unilm & GPT & GPT 3 \\  
   \midrule
甲&\multicolumn{5}{p{16cm}}{我不知您这个人眼力怎么样?}\\
乙&\multicolumn{5}{p{16cm}}{嗯，我眼神倒还行。}\\
甲&\multicolumn{5}{p{16cm}}{我看一看，两只小眼睛黑的乎地发亮。}\\
乙&\multicolumn{5}{p{16cm}}{什么叫小眼睛，您别看眼睛小，有神，看什么都看得清楚着呢!}\\
甲&\multicolumn{5}{p{16cm}}{什么都看得清楚?看个问题也尖锐?}\\
乙&\multicolumn{5}{p{16cm}}{那当然啦!}\\
甲&\multicolumn{5}{p{16cm}}{那您看看我这个人怎么样?}\\
乙&\multicolumn{5}{p{16cm}}{行，不错。}\\
甲&\multicolumn{5}{p{16cm}}{是说人品还是说长相?}\\
乙&\multicolumn{5}{p{16cm}}{从哪方面说都不错。}\\
\midrule
甲&是吗?嘿……&我是说你这么一个人，看见了吗?&您说一说。&有好人，说长相来也是有底线的。&那您看看我的这个人怎么样?\\ \hline
乙&看他还美了。&没有!&比方说吧，我长得跟鸭子似的，&那当然啦!&这个人，还行。\\ \hline
甲&不瞒您说，有人还把我比成花儿呢!&还有什么呀?&怎么?&你想一个人长得跟歪瓜裂枣似的，让大伙评评里头没有什么深度!&嗯，人品好、长相好、眼力好，我是一个完美的男人。\\ \hline
乙&是呀，比成什么花儿呀?&你看现在也没有别的地方。&鸭子嘴儿小，吃东西也没劲儿呀!&那我就说一条吧，这样的算术题，它绝对不能浅子了!&你是一个完美的男人?那你的女朋友呢?\\ \hline
甲&蒺藜狗子。&什么叫逮住?&哎哟!真是太好啦!&啊?您看这个标题，有大份儿好人性的、坏人做事没教养的。&我没有女朋友。\\ \hline
乙&啊，蒺藜狗子呀!&撞虫子上了。&鸭子嘴儿小，吃东西也没劲儿呀!&嘿，您真是猜着了人家不少朋友。&没有女朋友?你以前不是说你今年才28岁吗?\\ \hline
甲&这花儿怎么样?&危险性嘛?&对呀!&您就别谦虚了，我告诉你。&是啊，我今年才28岁。\\ \hline
乙&这不花儿，这是草。小枝小叶，浑身是刺，逮什么沾什么，谁见了谁讨厌，长得寒碜着哪!&为什么?&再往下说，我这个人特别爱美。&请问:这个标题，把名字改一改。&28岁了，没有女朋友？这不是很不正常吗?\\ \hline
甲&我听他们这么叫我，也不象是夸我。&因为它竖起来，鄙人往前走。&哦，您是女孩子吗?&怎么改?&不正常吗?在西方国家很正常的。\\ \hline
乙&根本就不是。&啊?&当然啦!&您的名字是这样改下来的吗?公共汽车，挤巴车两用那么点儿就可以了。&在西方国家很正常？那在中国呢?\\ 
\bottomrule 
   \end{tabular} 
    \caption{The raw script and generated scripts 12} 
    \label{tab:raw12} 
 \end{table*}


